Extreme Video Compression with Pre-trained Diffusion Models

Diffusion models have achieved remarkable success in generating high quality image and video data. More recently, they have also been used for image compression with high perceptual quality. In this paper, we present a novel approach to extreme video compression leveraging the predictive power of diffusion-based generative models at the decoder. The conditional diffusion model takes several neural compressed frames and generates subsequent frames. When the reconstruction quality drops below the desired level, new frames are encoded to restart prediction. The entire video is sequentially encoded to achieve a visually pleasing reconstruction, considering perceptual quality metrics such as the learned perceptual image patch similarity (LPIPS) and the Frechet video distance (FVD), at bit rates as low as 0.02 bits per pixel (bpp). Experimental results demonstrate the effectiveness of the proposed scheme compared to standard codecs such as H.264 and H.265 in the low bpp regime. The results showcase the potential of exploiting the temporal relations in video data using generative models. Code is available at: https://github.com/ElesionKyrie/Extreme-Video-Compression-With-Prediction-Using-Pre-trainded-Diffusion-Models-

==> alg_dec.tex <==
\begin{algorithm}[h]
    \caption{Decoding}\label{pseudocode_decode}
    \textbf{Input}: List of frame index $S$, List of frames $\mathcal{A}$ encoded using neural codec, \\
    Pre-trained generative model $G_\theta(\cdot),$
    Neural Image decoding method $\mathrm{Dec}(\cdot)$ \\
    \textbf{Parameters}: Length of video $T$, Lengths of generation windows $k$ and $j$\\
\textbf{Output}: List of reconstructed frames $\hat{\mathcal{A}}$\\
    \begin{algorithmic}[1]
        \STATE $\hat{\mathcal{A}} \gets \emptyset$
        \FOR{$i, v$ {\bfseries in} $\mathrm{enumerate}(S)$}
            \IF{ $S[i+1] - S[i] > 1$ }
                \STATE $f \gets S[i+1] - S[i]$, $round \gets f \mid j$, $res \gets f - round \times j$
                \FOR{$ n = 1$ {\bfseries to} $round$}
                    \STATE $l \gets \text{length of }\hat{\mathcal{A}}$
                    \STATE $\hat{\mathcal{A}} \gets \hat{\mathcal{A}} \cup [G_{\theta}(\hat{A} _{l-k \colon l})]$
                \ENDFOR
                \IF{$res > 0$}
                    \STATE $l \gets \text{length of }\hat{\mathcal{A}}$
                    \STATE $\hat{\mathcal{A}} \gets \hat{\mathcal{A}} \cup [G_{\theta}(\hat{A} _{l-k \colon l})][0\colon res]$
                \ENDIF
            \ELSE
                \STATE $\hat{\mathcal{A}} \gets \hat{\mathcal{A}} \cup [\mathrm{Dec}(\mathcal{A}[i])]$
            \ENDIF
        \ENDFOR
        \STATE $l \gets \text{length of }\hat{\mathcal{A}}$, $round \gets (T - l) \mid j$, $res \gets (T - l) - round \times j$
        \FOR{$ n = 1$ {\bfseries to} $round$}
            \STATE $l \gets \text{length of }\hat{\mathcal{A}}$
            \STATE $\hat{\mathcal{A}} \gets \hat{\mathcal{A}} \cup [G_{\theta}(\hat{A} _{l-k \colon l})]$
        \ENDFOR
        \IF{$res > 0$}
            \STATE $l \gets \text{length of }\hat{\mathcal{A}}$
            \STATE $\hat{\mathcal{A}} \gets \hat{\mathcal{A}} \cup [G_{\theta}(\hat{A} _{l-k \colon l})][0\colon res]$
        \ENDIF
    
%    \STATE $\hat{\mathcal{A}} \gets \hat{\mathcal{A}}[:T]$
    \STATE \textbf{return} $\hat{\mathcal{A}}$
    \end{algorithmic}
\end{algorithm}

==> figure.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.8\columnwidth]{framework.png}
\caption{\textbf{Method overview.} The core components of our proposed video compression framework include an alternative encoding at the encoder and generation at the decoder. The first few frames are encoded using a standard compression method. The following frames are generated using a pre-trained generative model at the receiver.  When the generation quality drops below the desired threshold, new frames are encoded to sustain the overall visual quality.}
\label{fig:framewrok}
\end{figure*}

==> figures_ieee.tex <==
\begin{figure*}[h]
\centering %表示居中
% \includegraphics[scale=1]{visual_result.png}
\includegraphics[scale=0.8]{fig2.pdf}
% [height=4.5cm]表示高度
%[width=9.5cm]表示宽度
%{city.png}表示eps格式的图片，名为111
\caption{\textbf{Visual comparison with state-of-the-art codec on Cityscape dataset.} We present the first 6 frames and last 3 frames between original video frames (top row), H.264 codec (second row) and the proposed compression scheme (bottom row). Both H.264 compression and the videos compressed by our model are controlled to have a BPP (bits per pixel) of 0.07.Our model utilizes the first two frames to autoregressively generate some following frames based on an LPIPS threshold of 0.16.}
%图片的名称
\label{visualResult}
%图片的标签，用于文章中的引用，注意到标签的数字与实际文章显示的数字可能不同
\end{figure*}


\begin{figure*}[h]
\centering %表示居中
\includegraphics[scale=0.8]{fig3.pdf}
% [height=4.5cm]表示高度
%[width=9.5cm]表示宽度
%{city.png}表示eps格式的图片，名为111
\caption{\textbf{Visual comparison with state-of-the-art codec on SMMNIST dataset.} We present the first 6 frames and last 3 frames between original video frames (top row), H.264 codec (second row) and the proposed compression scheme (bottom row). Both H.264 compression and the videos compressed by our model are controlled to have a BPP (bits per pixel) of 0.04,LPIPS threshold is 0.16. We generate frames conditioning on 5 frames. }
%图片的名称
\label{smm_visualResult}
%图片的标签，用于文章中的引用，注意到标签的数字与实际文章显示的数字可能不同
\end{figure*}







==> table.tex <==
% \begin{tabular}{c|c|c|c}
%       \toprule % from booktabs package
% \diagbox{Methods}{Metrics} & PSNR  ($\uparrow$)       & LPIPS ($\downarrow$)          & FVD ($\downarrow$)            \\
% \midrule % from booktabs package
% H.265                          & $22.44 \pm 2.18$ & $0.22 \pm 0.04$&  $3886.70\pm 1174.39 $  \\
% H.264                          &  $\bm {24.74}\pm2.48$  & $0.13 \pm 0.04$   &  $2414.48 \pm 830.35$\\
% Ours                   &  $23.70 \pm 2.47 $  &  $\bm{0.12}\pm 0.03$   &  $\bm{613.93}\pm 190.81 $  \\
%  \bottomrule % from booktabs package
%     \end{tabular}




% \begin{tabular}{c|c|c|c}
%       \toprule % from booktabs package
% \diagbox{Methods}{Metrics} & PSNR  ($\uparrow$)       & LPIPS ($\downarrow$)          & FVD ($\downarrow$)            \\
% \midrule % from booktabs package
% H.265                          & $22.44 \pm 2.18$ & $0.22 \pm 0.04$&  $3886.70\pm 1174.39 $  \\
% H.264                          &  $24.74\pm2.48$  & $0.13 \pm 0.04$   &  $2414.48 \pm 830.35$\\
% Ours                   &  $23.70 \pm 2.47 $  &  $0.12\pm 0.03$   &  $\bm{613.93}\pm 190.81 $  \\
% DCVC-DC &  $\bm {34.68 }\pm 2.01 $  &  $\bm{0.037}\pm0.02$   &  $745.86\pm 401.16 $  \\
% \bottomrule % from booktabs package
% \end{tabular}


\begin{tabular}{c|c|c|c}
      \toprule % from booktabs package
\diagbox{Methods}{Metrics} & PSNR  ($\uparrow$)       & LPIPS ($\downarrow$)          & FVD ($\downarrow$)            \\
\midrule % from booktabs package
H.265                          & $22.44 \pm 2.18$ & $0.22 \pm 0.04$&  $3886.70\pm 1174.39 $  \\
H.264                          &  $24.74\pm2.48$  & $0.13 \pm 0.04$   &  $2414.48 \pm 830.35$\\
Ours                   &  $24.37 \pm 2.57 $  &  $0.10\pm 0.03$   &  $\bm{737.96}\pm 274.48 $  \\
DCVC-DC &  $\bm {34.68 }\pm 2.01 $  &  $\bm{0.037}\pm0.02$   &  $745.86\pm 401.16 $  \\
\bottomrule % from booktabs package
\end{tabular}


